Leveraging Generative AI Models to Explore Human Identity

This paper attempts to explore human identity by utilizing neural networks in an indirect manner. For this exploration, we adopt diffusion models, state-of-the-art AI generative models trained to create human face images. By relating the generated human face to human identity, we establish a correspondence between the face image generation process of the diffusion model and the process of human identity formation. Through experiments with the diffusion model, we observe that changes in its external input result in significant changes in the generated face image. Based on the correspondence, we indirectly confirm the dependence of human identity on external factors in the process of human identity formation. Furthermore, we introduce \textit{Fluidity of Human Identity}, a video artwork that expresses the fluid nature of human identity affected by varying external factors. The video is available at https://www.behance.net/gallery/219958453/Fluidity-of-Human-Identity?.

==> newbib.tex <==
Benjamin W (2008 [1936]) The Work of Art in the Age of Its Technological Reproducibility, and Other Writings on Media, Cambridge: The Belknap Press of Harvard University Press. p.37

Walter Benjamin, “A Small History of Photography,” in One-Way Street and Other Writings, Trans. Jephoctt E. and Shorter K. (London: Lowe and Brydone, 1979), 243. (Originally published in German in 1931under the title Kleine Geschichte der Photographie).


Sartre, J. P.(2007), Existenalism is a Humanism, C. Macomber(trans.), New Haven & London: Yale Univ. Press page 20

@incollection{freud1983interpretation,
  title={The interpretation of dreams},
  author={Freud, Sigmund},
  booktitle={Literature and Psychoanalysis},
  pages={29--33},
  year={1983},
  publisher={Columbia University Press}
}

@article{deleuze1987introduction,
  title={Introduction: rhizome},
  author={Deleuze, Gilles and Guattari, F{\'e}lix},
  journal={A thousand plateaus: Capitalism and schizophrenia},
  volume={2},
  pages={3--25},
  year={1987},
  publisher={University of Minnesota Press Minneapolis}
}

(Assemblage)
Deleuze, Gilles and Félix Guattari, A Thousand Plateaus, Translated by Brian Massumi (Minneapolis: University of Minnesota Press,  1987), 399
